Effect of Adaptive Communication Support on LLM-powered Human-Robot Collaboration

Effective human-robot collaboration requires robot to adopt their roles and levels of support based on human needs, task requirements, and complexity. Traditional human-robot teaming often relies on a pre-determined robot communication scheme, restricting teamwork adaptability in complex tasks. Leveraging strong communication capabilities of Large Language Models (LLMs), we propose a Human-Robot Teaming Framework with Multi-Modal Language feedback (HRT-ML), a framework designed to enhance human-robot interaction by adjusting the frequency and content of language-based feedback. HRT-ML framework includes two core modules: a Coordinator for high-level, low-frequency strategic guidance, and a Manager for subtask-specific, high-frequency instructions, enabling passive and active interactions with human teammates. To assess the impact of language feedback in collaborative scenarios, we conducted experiments in an enhanced Overcooked environment with varying levels of task complexity (easy, medium, hard) and feedback frequency (inactive, passive, active, superactive). Our results show that as task complexity increases relative to human capabilities, human teammates exhibited a stronger preference towards robotic agents that can offer frequent, proactive support. However, when task complexities exceed the LLM's capacity, noisy and inaccurate feedback from superactive robotic agents can instead hinder team performance, as it requires human teammates to increase their effort to interpret and respond to a large number of communications, with limited performance return. Our results offer a general principle for robotic agents to dynamically adjust their levels and frequencies of communications to work seamlessly with humans and achieve improved teaming performance.

==> backup.tex <==
{\SH 
\section{Human-Robot Teaming Framework with Graph-Based Multi-Modal Language Feedback}

To provide adaptive language feedback in human-robot collaboration, HRT-ML leverages a Directed Acyclic Graph (DAG) to represent subtasks and its dependencies (e.g., finishing an onion soup) for human-robot collaboration. Based on the DAG,  HRT-ML includes three modules: the \textit{Coordinator}, the \textit{Manager}, and the \textit{Monitor}.  The \textit{Coordinator} leads high-level strategy discussions, generating an initial subtask graph, while the \textit{Manager} handles detailed subtask allocation based on finalized high-level coordination strategy DAG. \textit{Monitor} checks the status of the assigned subtask to both human and robot and updates the graph. 

\subsection{Subtask Graph for Human-Robot Collaboration}

We represent the collaboration goal as a dynamic directed acyclic graph (DAG) where nodes represent subtasks (e.g., \textit{pick onion}, \textit{cook onion}), and edges represent dependencies between tasks. Each edge is defined as \textit{(parent node,  node, cost)}, where the cost is calculated using an existing path planner using Depth First Search. Each node in the graph contains attributes for different coordination purposes:
\begin{itemize}
\item \textbf{Task id:} Each task gets a unique id, such that the LLM only needs to return the task id, and we can retrieve all other information based on the task id. 
\item \textbf{Task Type:} Categorized as \textit{Putting}, \textit{Getting}, or \textit{Operating}. There exist constraints when assigning different subtasks to robots or humans depending on their state, e.g., a robot that already held an onion can not execute any \textit{Getting} or \textit{Operating} tasks. 
\item \textbf{Status:} Represents the execution state, includes \textit{ready-to-execute}, \textit{executing}, \textit{success}, \textit{failure}, \textit{emergency}. The status of each subtask is considered when an LLM is prompted to assign subtasks for Humans and Robots. 
\item \textbf{Target Position:} Specifies a list of locations in the environment where the task can be performed. One subtask can be executed at multiple locations. This will enable humans and robots to explore additional collaboration strategies, such as the human placing an onion on an empty counter while the robot retrieves it.
\item \textbf{Notes:} The subtask node includes a notes attribute that captures human preferences or additional instructions (e.g., a Human prefers to perform picking up an onion; a Human is observed to be proficient at picking up onion.).
\item \textbf{Parent subtasks:} The parent subtasks indicate the prerequisite subtasks that are required to be \textit{success} before this subtask can be executed.
\item \textbf{Priority}: Priority is considered when assigning subtasks to humans and robots. It is calculated as the accumulated cost from the current node to the sink (termination) node. 
\item \textbf{Running time}: The running time acts as a counter, recording the duration for which the robot has been assigned to this subtask. 
\end{itemize}
The subtask graph enables the robot to translate language-based coordination into modifications within the graph, helping the LLM organize conversations and align its knowledge with the human's.
\subsection{Coordinator}

The \textit{Coordinator} of the robot is responsible for designing overall collaboration strategies and discussing them with the human partner. The initial subtask graph is generated using a one-shot LLM prompt (\appref{app:prompt-gen}), incorporating recipe and kitchen layout information. We then implement a dialog-based graph modification, which can be initiated by the robot at a low frequency with the corresponding prompt (\appref{app:prompt-gen})  (active mode / superactive mode described in \secref{sec: modes} or proactively by the human through language-based feedback. The coordination process can be divided into the following decision tree:
\begin{itemize}
    \item The robot first identifies the type of human request, which falls into one of three categories; if it is unsure, it will further ask a human to clarify.
    \begin{itemize}
        \item \textit{Subtask Graph Structure Change:} The human expresses thoughts on how to complete the overall task. This may involve adding nodes, further decomposing a subtask for human and robot execution, or correcting incorrect graph dependencies. For example, based on the environment (\figref{fig.environment} B), one of the possible coordination strategies is that the robot can place the onion at location (5, 2), and the human (blue agent) should focus on picking up onions at (5, 2).

        \item \textit{Subtask Attribute Change:} The human specifies preferences for subtask assignments. For example, based on the environment (\figref{fig.environment} B), a human says that he would like to handle picking up onions and dishes as well as putting them on the counter (5, 2) and (6, 2).

        \item \textit{Temporary Subtask Assignment:} The human is not designing an overall collaboration strategy but instead requests the robot to execute a specific temporary subtask. For example, if the robot is blocking the human's path while they attempt to put an onion in the pot, the human may instruct the robot to move to a specific position. 
    \end{itemize}
    \item After identifying the type of coordination, the subtask graph is updated using the prompts shown in Appendix \ref{app:prompt-gen} for each category.
\end{itemize}

During these coordination discussions, the game remains paused until the human concludes the conversation. 
 
\subsection{Manager}

The \textit{Manager} is responsible for real-time subtask allocation based on the information from the subtask graph and subtask status monitoring. 

\subsubsection{Subtask Allocation}
The \textit{Manager} were first asked to analyze the current state of humans and robots along with the list of subtasks that are ready to execute return by the subtask graph. The prompt (\appref{app:prompt-manager}) explicitly instructs the robot to consider task priorities and types based on the current state, as well as human-reported preferences for each subtask. Besides subtask assignments, the \textit{Manager} is also prompted to generate language instructions to guide the human in executing their assigned subtasks toward the final goal. This feedback is selectively presented to the human based on the feedback mode described in \secref{sec: modes}. 

\subsubsection{Subtask status update}
The \textit{Manager} will be triggered to evaluate the current executing task to update the status given the human and robot action trajectory when an \textit{Interact} action is executed (Prompt details can be found in \appref{app:prompt-manager}). Once a subtask is identified as \textit{success}, the subtask nodes without unresolved dependencies will be marked as \textit{ready-to-execute}, while others remain \textit{not-ready} until their prerequisites are completed. 

\subsection{Action Planner}

Once a subtask (target location) is assigned, the robot uses a greedy planner based on Depth First Search (DFS) to determine the sequence of atomic actions required to complete the task. The planner computes the optimal path with the lowest action cost, considering the current environment layout and agent states.



\subsection{Multi-Modal Feedback}
\label{sec: modes}
Building on the graph-based HRT-ML framework, we introduce four levels of language feedback:
\begin{itemize}
\item \textit{Inactive Feedback Agent (IFA):} The IFA collaborates without language communication. Only the \textit{Manager} generates subtasks for the greedy planner.
\item \textit{Passive Feedback Agent (PFA):} The PFA provides feedback only upon human request. The human leads, while the agent responds passively. If no requests are made, the PFA behaves like an IFA.
\item \textit{Active Feedback Agent (AFA):} The AFA acts as a peer, providing feedback proactively at low frequency (e.g., every 20 seconds) by analyzing the conversation history and suggesting strategies.
\item \textit{Superactive Feedback Agent (SFA):} The SFA acts as a supervisor, providing continuous, frequent guidance on every subtask.
\end{itemize}

The subtask graph enables adaptive feedback by allowing agents to dynamically update tasks, preferences, and dependencies based on human input and environment changes. The graph’s structure provides a clear representation of task progress, ensuring efficient collaboration and transparent communication.

}


